Automatic Testing With Reusable Adversarial Agents

Autonomous systems such as self-driving cars and general-purpose robots are safety-critical systems that operate in highly uncertain and dynamic environments. We propose an interactive multi-agent framework where the system-under-design is modeled as an ego agent and its environment is modeled by a number of adversarial (ado) agents. For example, a self-driving car is an ego agent whose behavior is influenced by ado agents such as pedestrians, bicyclists, traffic lights, road geometry etc. Given a logical specification of the correct behavior of the ego agent, and a set of constraints that encode reasonable adversarial behavior, our framework reduces the adversarial testing problem to the problem of synthesizing controllers for (constrained) ado agents that cause the ego agent to violate its specifications. Specifically, we explore the use of tabular and deep reinforcement learning approaches for synthesizing adversarial agents. We show that ado agents trained in this fashion are better than traditional falsification or testing techniques because they can generalize to ego agents and environments that differ from the original ego agent. We demonstrate the efficacy of our technique on two real-world case studies from the domain of self-driving cars.

==> sections/grid_world_case.tex <==
\subsection{Gridworld case}

The model is a gridworld with two agents. The ado agent is trying to
``catch'' the ego agent. The ado agent successfully catches the ego
agent if they arrive in the same cell. The actions available for both
agents are: (up, down, left, right).
At each time step, ego and ado observe each others current position,
then ego moves first ado moves after the ego moves.  (interleaved
concurrency)

The state for the ego agent is the coordinate of the ado agent. Policy
for ego agent is it will calculate the direction that is furthest from
the ado agent, break the tie by choosing horizontal direction first.
If the action is hitting into the wall, the ego agent will try the
other decomposed direction corresponding to the vector that connect
ego and ado agent, if the second try fails also, then the ego agent
will stay still. 

Use a four 2x2 grid world to justify the ego agent is not too dumb. 

% The policy for vanila ado agent is the same as ego agent. 

The state space for a DQN based ado agent is coordinate of the ego
agent and their relative distance and direction.

The episode ends when two agents land in a same coordinate or time
out.


We first show the case when all agents have step size 1. Then we shall
the case when ado agent can have step size larger than ego agent.


